Enhancing Taxonomy Completion with Concept Generation via Fusing Relational Representations

Automatic construction of a taxonomy supports many applications in e-commerce, web search, and question answering. Existing taxonomy expansion or completion methods assume that new concepts have been accurately extracted and their embedding vectors learned from the text corpus. However, one critical and fundamental challenge in fixing the incompleteness of taxonomies is the incompleteness of the extracted concepts, especially for those whose names have multiple words and consequently low frequency in the corpus. To resolve the limitations of extraction-based methods, we propose GenTaxo to enhance taxonomy completion by identifying positions in existing taxonomies that need new concepts and then generating appropriate concept names. Instead of relying on the corpus for concept embeddings, GenTaxo learns the contextual embeddings from their surrounding graph-based and language-based relational information, and leverages the corpus for pre-training a concept name generator. Experimental results demonstrate that GenTaxo improves the completeness of taxonomies over existing methods.

==> Tables/baseline_exp2.tex <==
\begin{table}[t]
\caption{Comparison of OntoGen against the baseline methods on ontology completion task (in \%). TaxoExpan shows the strongest performance on IE-based baselines on precision, recall and F1-score. Our OntoGen achieves the SOTA on recall and F1-score than IE-based models.}
\label{tab:baseline_exp2}
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c}{} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\ \midrule
\multicolumn{1}{l}{\textbf{HiExpan}} & 17.77 & 5.66 & 8.59 \\
\multicolumn{1}{l}{\textbf{TaxoExpan}} &  \underline{\textbf{26.87}} & 11.79 & 16.39 \\
\multicolumn{1}{l}{\textbf{STEAM}} & 26.05 & 11.23 & 15.69 \\
\multicolumn{1}{l}{\textbf{Graph2Taxo}} & 26.13 & 10.35 & 14.83 \\  \midrule
% \multicolumn{1}{c}{\textbf{Upper Bound}} & 39.60 & 100.00 & 29.75 \\ \midrule
\multicolumn{1}{l}{\textbf{\textsc{OntoGen}}} & 21.47 & \underline{\textbf{17.10}} & \underline{\textbf{19.03}} \\ \bottomrule
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
\end{tabular}
\end{table}

==> Tables/data_stat_new.tex <==
\begin{table*}[h]
\caption{Data statistics. $|\mathcal{N}|$ and $|\mathcal{E}|$ are the number of concepts and edges in the six taxonomies, respectively. $|\mathcal{D}|$ is the depth of the taxonomy.}
\begin{tabular}{c|cccccc}
\hline
 & $|\mathcal{N}|$ & $|\mathcal{E}|$ & $|\mathcal{D}|$ & \textbf{\# of Concepts in corpus} & \textbf{\# unique words} & \textbf{\# word in vocabulary} \\ \hline
\textbf{MeSH} & 9711 & 30191 & 15 & 8517 & 4875 & 4875 \\
\textbf{MAG-CS} & 17384 & 53250 & 6 & 12433 & 5699 & 5668 \\
\textbf{OS} & 984 & 1041 & 4 & 577 & 967 & 958 \\
\textbf{Drone} & 254 & 518 & 4 & 207 & 247 & 237 \\
\textbf{SemEval-Sci} & 429 & 452 & 8 & 393 & 573 & 573 \\
\textbf{SemEval-Env} & 261 & 261 & 6 & 223 & 317 & 317 \\ \hline
\end{tabular}
\label{tab:stat}
\end{table*}

\begin{table*}[h]
\caption{Data statistics. $|\mathcal{N}|$ and $|\mathcal{E}|$ are the number of concepts and edges in the six taxonomies, respectively. $|\mathcal{D}|$ is the depth of the taxonomy.}
\begin{tabular}{c|cccccc}
\hline
 & $|\mathcal{N}|$ & $|\mathcal{E}|$ & $|\mathcal{D}|$ & \textbf{\# of Concepts in corpus} & \textbf{\# unique words} & \textbf{\# word in vocabulary} \\ \hline
\textbf{MeSH} & 29758 & 40186 & 15 & 14164 & 22367  & 22193 &  \\
\textbf{MAG-CS} & 29484 & 46144 & 6 & 18338 & 16398 & 13914 \\
\textbf{OS} & 984 & 1041 & 4 & 577 & 967 & 958 \\
\textbf{Drone} & 263 & 528 & 4 & 207 & 247 & 237 \\
\textbf{SemEval-Sci} & 429 & 452 & 8 & 393 & 573 & 573  \\
\textbf{SemEval-Env} & 261 & 261 & 6 & 223 & 317 & 317 \\ \hline
\end{tabular}
\label{tab:stat-ori}
\end{table*}

==> Tables/data_statistics_old.tex <==
\begin{table}[t]
\caption{Data statistics. $|\mathcal{N}|$ and $|\mathcal{E}|$ are the number of nodes and edges in the MeSH ontology, respectively. $|\mathcal{D}|$ is the depth of the ontology. $|\mathcal{T}|$ indicates the number of concepts.}
\begin{tabular}{lrrrr}
\toprule
 & $|\mathcal{N}|$ & $|\mathcal{E}|$ & $|\mathcal{D}|$ & $|\mathcal{T}|$ \\ \midrule
\textbf{Train} & 14,624 & 20,609 & 15 & 5,827\\
\textbf{Dev} & 6,752 & 6,754 & 15 & 1,942 \\
\textbf{Test} & 7,010 & 7,052 & 15 & 1,942 \\ \midrule
\textbf{All} & 29,758 & 80,372 & 15 & 29,758 \\ \bottomrule
\end{tabular}
\label{tab:stat}
\end{table}


==> Tables/encoder_combination.tex <==
\begin{table}[h]
\caption{Encoder selection for three most common relation among entities in ontology. We investigate the best combination between graph-based context encoder (Graph) and sentence-based context encoder (Sent) for each relation. 
The results shows that for Parent-Child (1-hop) relation, sentence-based context encoder is the most effective. For multi-hop relations (Sibling-Sibling and Grandparent-Grandchild), the fusion of graph-based context encoder and sentence-based context encoder is the most suitable way.  }
\label{tab:encoders_combination}
\begin{tabular}{lccc}
\toprule
\textbf{1-hop} & \textbf{F1} & \textbf{F1-Uni} & \textbf{F1-Multi} \\ \midrule
\textbf{Graph} & 4.86 & 5.60 & 4.71 \\
\textbf{Sent} & \underline{\textbf{16.83}} & 16.26 & \underline{\textbf{16.82}} \\
\textbf{Graph+Sent} & 16.49 &\underline{\textbf{17.32}} & 16.27 \\ \bottomrule
\toprule
\textbf{2-hop} & \textbf{F1} & \textbf{F1-Uni} & \textbf{F1-Multi} \\ \midrule
\textbf{Graph} & 7.40 & 6.40 & 7.52 \\
\textbf{Sent} & 13.59 & 12.79 & 13.63 \\
\textbf{Graph+Sent} & \underline{\textbf{14.92}} & \underline{\textbf{14.13}} & \underline{\textbf{14.98}} \\ \bottomrule
\toprule
\textbf{Grandparent-Grandchild} & \textbf{F1} & \textbf{F1-Uni} & \textbf{F1-Multi} \\ \midrule
\textbf{Graph} & 3.35 & 3.73 & 3.27 \\
\textbf{Sent} & 10.39 & 9.87 & 10.41 \\
\textbf{Graph+Sent} & \underline{\textbf{12.34}} & \underline{\textbf{13.06}} & \underline{\textbf{12.14}} \\ \bottomrule
\end{tabular}
\end{table}
